A Dataset for Semantic Segmentation in the Presence of Unknowns

Before deployment in the real-world deep neural networks require thorough evaluation of how they handle both knowns, inputs represented in the training data, and unknowns (anomalies). This is especially important for scene understanding tasks with safety critical applications, such as in autonomous driving. Existing datasets allow evaluation of only knowns or unknowns - but not both, which is required to establish "in the wild" suitability of deep neural network models. To bridge this gap, we propose a novel anomaly segmentation dataset, ISSU, that features a diverse set of anomaly inputs from cluttered real-world environments. The dataset is twice larger than existing anomaly segmentation datasets, and provides a training, validation and test set for controlled in-domain evaluation. The test set consists of a static and temporal part, with the latter comprised of videos. The dataset provides annotations for both closed-set (knowns) and anomalies, enabling closed-set and open-set evaluation. The dataset covers diverse conditions, such as domain and cross-sensor shift, illumination variation and allows ablation of anomaly detection methods with respect to these variations. Evaluation results of current state-of-the-art methods confirm the need for improvements especially in domain-generalization, small and large object segmentation.

==> tables/cvpr_reb_metrics_in-domain.tex <==




















\begin{table}[ht]
\centering
\footnotesize
\setlength{\tabcolsep}{2.3pt}
\begin{tabular}{lcccccc}
\toprule


\multicolumn{7}{c}{Road Anomaly} \\
\midrule

\multirow{2}{*}{Method} & \multicolumn{3}{c}{Static} & \multicolumn{3}{c}{Temporal}\\

\cmidrule(lr){2-4}
\cmidrule(lr){5-7}

 {} &  
\multicolumn{1}{c}{mF1 $\uparrow$} & \multicolumn{1}{c}{sIoU $\uparrow$} & \multicolumn{1}{c}{PPV $\uparrow$} &  \multicolumn{1}{c}{mF1 $\uparrow$} & \multicolumn{1}{c}{sIoU $\uparrow$} & \multicolumn{1}{c}{PPV $\uparrow$}  \\ 


\midrule
 JSRNet  & 3.2/1.7 & 13.8/14.6 & 8.2/3.2 & 1.2/1.2 & 12.0/13.5 & 4.4/2.6 \\
 PixOOD & 1.8/1.9 & 15.6/27.5 & 13.4/7.6 & 1.4/1.4 & 14.1/24.7 & 7.8/3.7 \\%[0.3em]
 RbA    & 11.2/15.3 & 28.5/36.7 & 19.9/18.2 & 5.7/10.7 & 17.5/25.6 & 12.4/17.8 \\
 RbA$^\dagger$    & 9.6/20.2 & 33.2/36.9 & 15.5/25.7 & 5.3/11.2 & 19.9/21.6 & 11.9/23.9 \\
 EAM$^\dagger$    & 21.5/20.7 &	30.4/39.1 &	25.2/23.0 &	10.6/14.7 &	25.9/27.8 &	13.5/20.2 \\


\bottomrule


\multicolumn{7}{c}{Road Obstacle} \\
\midrule

\multirow{2}{*}{Method} 
&  \multicolumn{3}{c}{Static} & \multicolumn{3}{c}{Temporal}\\

\cmidrule(lr){2-4}
\cmidrule(lr){5-7}

 {} &  
\multicolumn{1}{c}{mF1 $\uparrow$} & \multicolumn{1}{c}{sIoU $\uparrow$} & \multicolumn{1}{c}{PPV $\uparrow$} &  \multicolumn{1}{c}{mF1 $\uparrow$} & \multicolumn{1}{c}{sIoU $\uparrow$} & \multicolumn{1}{c}{PPV $\uparrow$}  \\ 


\midrule
 JSRNet    & 31.2/24.3 & 55.4/62.4 & 33.2/23.8 & 11.5/18.6 & 25.4/45.1 & 28.1/26.6 \\
 PixOOD  & 28.0/27.9 & 58.9/64.6 & 27.3/22.9 & 33.6/28.2 & 50.5/53.7 & 35.8/27.6 \\
  RbA        & 25.6/29.5 & 37.7/51.7 & 38.6/30.1 & 13.7/22.5 & 26.0/41.8 & 25.1/27.4 \\
  RbA$^\dagger$    & 17.5/36.9 & 40.9/50.9 & 24.6/40.0 & 9.3/23.5 & 26.6/39.1 & 18.0/31.9 \\
 EAM$^\dagger$    & 36.3/41.4 &	35.5/56.7 &	47.9/38.7 &	23.6/27.9 &	30.8/48.4 &	32.4/26.8 \\
\bottomrule
\end{tabular}
\vspace{-3mm}
\caption{Component-level metrics for road anomaly (top) and  obstacle (bottom) tracks in the form \textbf{cross-domain/in-domain}.
\textdagger indicates training with OOD data.}
\vspace{-5mm}
\label{tab:cd_os}
\end{table}%







